Sum-of-Squares proofs of logarithmic Sobolev inequalities on finite Markov chains

Logarithmic Sobolev inequalities are a fundamental class of inequalities that play an important role in information theory. They play a key role in establishing concentration inequalities and in obtaining quantitative estimates on the convergence to equilibrium of Markov processes. More recently, deep links have been established between logarithmic Sobolev inequalities and strong data processing inequalities. In this paper we study logarithmic Sobolev inequalities from a computational point of view. We describe a hierarchy of semidefinite programming relaxations which give certified lower bounds on the logarithmic Sobolev constant of a finite Markov operator, and we prove that the optimal values of these semidefinite programs converge to the logarithmic Sobolev constant. Numerical experiments show that these relaxations are often very close to the true constant even for low levels of the hierarchy. Finally, we exploit our relaxation to obtain a sum-of-squares proof that the logarithmic Sobolev constant is equal to half the Poincar\'e constant for the specific case of a simple random walk on the odd $n$-cycle, with $n\in\{5,7,\dots,21\}$. Previously this was known only for $n=5$ and even $n$.

==> lsi.tex <==
%!TEX root = paper.tex

In this subsection, we will mention some fundamental results and examples in the theory of logarithmic Sobolev inequalities for Markov chains on finite state spaces. 
We will build on what was already covered in section \ref{sec:intro}.
The content is mostly extracted from the expository paper \cite{P.Diaconis1996}, as well as from \cite{Saloff-Coste1997} and \cite{Montenegro2006}.

Consider a Markov kernel $K$ on a finite state space $\mathcal{X}=\{1, \dots, n\}$, with log-Sobolev constant $\alpha$ and Poincar\'e constant $\lambda$.
It is not \emph{a priori} obvious that $\alpha$ is positive.
This is a consequence of the following result.
\begin{thm}\cite[Theorem~2.2.3]{Saloff-Coste1997}\label{non_constant}
    Let $K$ be an irreducible Markov kernel. Then $2\alpha\le \lambda$.
    Moreover, if $2\alpha < \lambda$, then there exists a non-constant, elementwise positive $u\in\R_+^n$ such that $\alpha=\frac{\mathcal{E}(u,u)}{\Ent_\pi[u]}$, and satisfying
    \begin{equation}\label{grad-cond}
        2u\log u - 2u\log\norm{u}_\pi -\alpha\inv(I-K)u=0.
    \end{equation}
\end{thm}
The next result shows that log-Sobolev inequalities ``tensorize'' --- a useful tool for obtaining the log-Sobolev constants of larger chains from those of smaller chains.
\begin{lemma}\cite[Lemma~2.2.11]{Saloff-Coste1997}\label{product}
    Consider $(K_i, \pi_i)$, $i=1,\dots,d$, Markov chains on finite spaces $\mathcal{X}_i$ with spectral gaps $\lambda_i$ and log-Sobolev constants $\alpha_i$.
    Let $\mu$ be a positive distribution on $1,\dots, d$.
    Consider the product chain on $\mathcal{X}_1\times\dots\times\mathcal{X}_d$, which at each step chooses a coordinate $i$ randomly according to $\mu$ and takes a step in that coordinate according to $K_i$.
    This chain has Markov kernel
    \[K_\mu = \sum_{i=1}^d \mu_i I\otimes\dots\otimes K_i\otimes\dots\otimes I.\]
    The log-Sobolev and Poincar\'e constants of this product chain are given by
    \[\alpha = \min_{i=1,\ldots,d} \mu_i\alpha_i \qquad \lambda = \min_{i=1,\ldots,d} \mu_i\lambda_i.\]
\end{lemma}

Even on finite state spaces, the log-Sobolev constants of only a few Markov chains are known.
These include all two-point chains, certain specific chains on 3-point and 4-point spaces, and the simple random walk on complete graphs and on the $n$-cycle $C_n$ when $n$ is even and when $n=5$.
For concreteness, we discuss some of these (very briefly) in the examples below.

\begin{example}\label{two-state-ind}
    Consider the two state chain with kernel $K=\begin{psmallmatrix}\theta & 1-\theta\\ \theta &1-\theta \end{psmallmatrix}$ for $0<\theta\le\half$, and stationary distribution $\pi_1=\theta, \pi_2=1-\theta$.
    We have 
    \[\alpha = \frac{1-2\theta}{\log\left(\frac{1-\theta}{\theta}\right)}.\]
    For the symmetric case $\theta=\half$, the right hand side is replaced by its limit, which is $\half$ (note that $\lambda=1$ for this chain).
    It can be deduced that the simple random walk on $\Z_2$ has log-Sobolev constant $1$.
    Using Lemma \ref{product}, it follows that the log-Sobolev constant of the hypercube $\Z_2^d$ is $1/d$.
    \begin{figure}[htbp]
        \centering
        \tikzfig{png/2state}
        \caption{The two-state chain of Example \ref{two-state-ind}.}\label{fig:2state}
    \end{figure}
\end{example}

\begin{example}\label{many-state-ind}
    Let $\pi$ be a positive distribution on a finite space, and consider the chain with kernel $K_{ij}=\pi_j$ and stationary distribution $\pi$.
    Write $\pi_*=\min_i\pi_i$.
    Then \[\alpha = \frac{1-2\pi_*}{\log\left(\pi_*\inv-1\right)}.\]
    It can be deduced that the log-Sobolev constant for the simple random walk on the complete graph on $n$ nodes is $\frac{n-2}{(n-1)\log\left(n-1\right)}$.
    This is different from $\lambda/2$ for $n>2$.
\end{example}

\begin{example}\label{cycle-ex}
    Consider the simple random walk on the $n$-cycle, with kernel $K_{i,i\pm1 \text{ (mod }n)} = 1/2$.
    For $n$ even and for $n=5$, one has 
    \[2\alpha = \lambda = 1 - \cos(2\pi/n).\]
    Note that $C_2\cong\Z_2$ and $C_4\cong\Z_2^2$, so for $n=2, 4$, this comes from Example \ref{two-state-ind}.
    The general even case was proved in \cite{Chen2003}, and the $n=5$ case was proved in \cite{Chen2008} by collapsing the chain to a 3-point stick.
    It is conjectured (\cite{Chen2008}) that equality holds for odd $n>5$ too.
\end{example}



As demonstrated in Example \ref{two-state-ind}, it is possible to obtain log-Sobolev constants for more complicated chains from simpler chains by considering product chains (Lemma \ref{product}), and by comparison arguments.
Therefore it remains of interest to compute, or at least bound, the log-Sobolev constants of small chains.



==> png/padeapprox.tex <==
\begin{tikzpicture}[]
\begin{axis}[legend pos = {south east}, title = {$\left\vert\frac{\overline{r_m}(t)}{\log(t)}-1\right\vert$}, ymax = {10000}, ymode = {log}, xlabel = {$t$}, ymin = {1.0000000000000008e-16}]\addplot+ [mark = {none}]coordinates {
(0.0, NaN)
(0.12121212121212122, 0.034699475328781565)
(0.24242424242424243, 0.00666664274548342)
(0.36363636363636365, 0.0014365800039234577)
(0.48484848484848486, 0.0002930166817126989)
(0.6060606060606061, 4.884567992925131e-5)
(0.7272727272727273, 5.249998765886483e-6)
(0.8484848484848485, 1.961639001719318e-7)
(0.9696969696969697, 4.585748291358526e-11)
(1.0909090909090908, 8.367499435435268e-9)
(1.2121212121212122, 4.4453685909672123e-7)
(1.3333333333333333, 3.334991608341338e-6)
(1.4545454545454546, 1.2513570435918365e-5)
(1.5757575757575757, 3.293179718664276e-5)
(1.696969696969697, 6.994766560778624e-5)
(1.8181818181818181, 0.0001288186098558387)
(1.9393939393939394, 0.00021439521055820814)
(2.0606060606060606, 0.0003309634941242215)
(2.1818181818181817, 0.0004821853656583842)
(2.303030303030303, 0.0006710992041276726)
(2.4242424242424243, 0.0009001546926903043)
(2.5454545454545454, 0.0011712651058331427)
(2.6666666666666665, 0.0014858666218878825)
(2.787878787878788, 0.0018449784340050463)
(2.909090909090909, 0.002249260137915317)
(3.0303030303030303, 0.0026990645752558223)
(3.1515151515151514, 0.003194485354839498)
(3.272727272727273, 0.003735398895581701)
(3.393939393939394, 0.004321501188444046)
(3.515151515151515, 0.004952339661199587)
(3.6363636363636362, 0.0056273406136260655)
(3.757575757575758, 0.0063458327131909)
(3.878787878787879, 0.007107067028467586)
(4.0, 0.00791023404571406)
(4.121212121212121, 0.008754478073349559)
(4.242424242424242, 0.009638909395476632)
(4.363636363636363, 0.010562614492699475)
(4.484848484848484, 0.011524664608142589)
(4.606060606060606, 0.012524122899784966)
(4.7272727272727275, 0.01356005038727279)
(4.848484848484849, 0.014631510872305903)
(4.96969696969697, 0.015737574986273227)
(5.090909090909091, 0.01687732349671507)
(5.212121212121212, 0.01804984998515619)
(5.333333333333333, 0.019254262992418017)
(5.454545454545454, 0.020489687713450378)
(5.575757575757576, 0.021755267311662368)
(5.696969696969697, 0.0230501639124186)
(5.818181818181818, 0.024373559326552927)
(5.9393939393939394, 0.025724655547234174)
(6.0606060606060606, 0.02710267505709286)
(6.181818181818182, 0.02850686097704055)
(6.303030303030303, 0.029936477083541427)
(6.424242424242424, 0.031390807717104424)
(6.545454545454546, 0.032869157601360076)
(6.666666666666667, 0.03437085158918031)
(6.787878787878788, 0.03589523434982039)
(6.909090909090909, 0.03744167000894556)
(7.03030303030303, 0.039009541751589966)
(7.151515151515151, 0.0405982513965548)
(7.2727272727272725, 0.04220721894943385)
(7.393939393939394, 0.04383588214031734)
(7.515151515151516, 0.04548369595127707)
(7.636363636363637, 0.0471501321378937)
(7.757575757575758, 0.04883467874839762)
(7.878787878787879, 0.05053683964339047)
(8.0, 0.05225613401859804)
(8.121212121212121, 0.053992095932668877)
(8.242424242424242, 0.05574427384166633)
(8.363636363636363, 0.05751223014157747)
(8.484848484848484, 0.059295540719887546)
(8.606060606060606, 0.06109379451705829)
(8.727272727272727, 0.06290659309852614)
(8.848484848484848, 0.06473355023769496)
(8.969696969696969, 0.06657429151025043)
(9.090909090909092, 0.0684284538999946)
(9.212121212121213, 0.07029568541632603)
(9.333333333333334, 0.07217564472337895)
(9.454545454545455, 0.07406800078079342)
(9.575757575757576, 0.07597243249601181)
(9.696969696969697, 0.07788862838796001)
(9.818181818181818, 0.07981628626193542)
(9.93939393939394, 0.08175511289548608)
(10.06060606060606, 0.08370482373504758)
(10.181818181818182, 0.08566514260308222)
(10.303030303030303, 0.08763580141545392)
(10.424242424242424, 0.08961653990875962)
(10.545454545454545, 0.09160710537732875)
(10.666666666666666, 0.09360725241960617)
(10.787878787878787, 0.09561674269362304)
(10.909090909090908, 0.09763534468126417)
(11.030303030303031, 0.09966283346104565)
(11.151515151515152, 0.1016989904891091)
(11.272727272727273, 0.10374360338815915)
(11.393939393939394, 0.10579646574405589)
(11.515151515151516, 0.10785737690979844)
(11.636363636363637, 0.10992614181662969)
(11.757575757575758, 0.11200257079200243)
(11.878787878787879, 0.11408647938415971)
(12.0, 0.11617768819307618)
};
\addlegendentry{$m=2$}
\addplot+ [mark = {none}]coordinates {
(0.0, NaN)
(0.12121212121212122, 0.008333514451194807)
(0.24242424242424243, 0.0007789826417184416)
(0.36363636363636365, 8.815138714449199e-5)
(0.48484848484848486, 9.340232461599966e-6)
(0.6060606060606061, 7.500745883528476e-7)
(0.7272727272727273, 3.2681709144792114e-8)
(0.8484848484848485, 3.2501226130289315e-10)
(0.9696969696969697, 2.7059551046187135e-15)
(1.0909090909090908, 3.869801596418055e-12)
(1.2121212121212122, 1.001230589584535e-9)
(1.3333333333333333, 1.672787701712912e-8)
(1.4545454545454546, 1.0599157074791231e-7)
(1.5757575757575757, 4.088624743327636e-7)
(1.696969696969697, 1.168686056351837e-6)
(1.8181818181818181, 2.7364400996279958e-6)
(1.9393939393939394, 5.561630408048416e-6)
(2.0606060606060606, 1.017536319346336e-5)
(2.1818181818181817, 1.7170205291501944e-5)
(2.303030303030303, 2.7179922105298857e-5)
(2.4242424242424243, 4.0860883218836356e-5)
(2.5454545454545454, 5.887600156420264e-5)
(2.6666666666666665, 8.188148157889475e-5)
(2.787878787878788, 0.00011051630695606918)
(2.909090909090909, 0.000145394218119163)
(3.0303030303030303, 0.00018709785207943002)
(3.1515151515151514, 0.00023617470069504432)
(3.272727272727273, 0.00029313456005094026)
(3.393939393939394, 0.000358448176678278)
(3.515151515151515, 0.00043254683549568193)
(3.6363636363636362, 0.0005158226738373791)
(3.757575757575758, 0.0006086295427914532)
(3.878787878787879, 0.0007112842698519821)
(4.0, 0.0008240682052234361)
(4.121212121212121, 0.0009472289580459189)
(4.242424242424242, 0.0010809822487411597)
(4.363636363636363, 0.0012255138200685755)
(4.484848484848484, 0.0013809813628114641)
(4.606060606060606, 0.00154751642279345)
(4.7272727272727275, 0.0017252262645536622)
(4.848484848484849, 0.0019141956738760093)
(4.96969696969697, 0.0021144886867852995)
(5.090909090909091, 0.0023261502368910766)
(5.212121212121212, 0.0025492077162463937)
(5.333333333333333, 0.0027836724474399797)
(5.454545454545454, 0.003029541066576885)
(5.575757575757576, 0.0032867968182400033)
(5.696969696969697, 0.0035554107646009877)
(5.818181818181818, 0.003835342911601196)
(5.9393939393939394, 0.004126543255642739)
(6.0606060606060606, 0.004428952754575023)
(6.181818181818182, 0.004742504226949652)
(6.303030303030303, 0.005067123183595676)
(6.424242424242424, 0.0054027285955803766)
(6.545454545454546, 0.005749233602540154)
(6.666666666666667, 0.0061065461652822705)
(6.787878787878788, 0.006474569666394636)
(6.909090909090909, 0.006853203462462184)
(7.03030303030303, 0.007242343391300017)
(7.151515151515151, 0.007641882237434412)
(7.2727272727272725, 0.008051710158886885)
(7.393939393939394, 0.008471715078116643)
(7.515151515151516, 0.00890178303981291)
(7.636363636363637, 0.009341798538037308)
(7.757575757575758, 0.00979164481506405)
(7.878787878787879, 0.01025120413409004)
(8.0, 0.010720358027839754)
(8.121212121212121, 0.011198987524947045)
(8.242424242424242, 0.011686973355856263)
(8.363636363636363, 0.01218419613985535)
(8.484848484848484, 0.012690536554737605)
(8.606060606060606, 0.013205875490476202)
(8.727272727272727, 0.013730094188184338)
(8.848484848484848, 0.014263074365546524)
(8.969696969696969, 0.014804698329814112)
(9.090909090909092, 0.01535484907936057)
(9.212121212121213, 0.01591341039474005)
(9.333333333333334, 0.016480266920093137)
(9.454545454545455, 0.017055304235699793)
(9.575757575757576, 0.017638408922404186)
(9.696969696969697, 0.018229468618579808)
(9.818181818181818, 0.01882837207026306)
(9.93939393939394, 0.019435009175016477)
(10.06060606060606, 0.020049271020053498)
(10.181818181818182, 0.020671049915109426)
(10.303030303030303, 0.021300239420497472)
(10.424242424242424, 0.02193673437077439)
(10.545454545454545, 0.022580430894378438)
(10.666666666666666, 0.02323122642960361)
(10.787878787878787, 0.023889019737219876)
(10.909090909090908, 0.02455371091004202)
(11.030303030303031, 0.025225201379716365)
(11.151515151515152, 0.02590339392097501)
(11.272727272727273, 0.026588192653594394)
(11.393939393939394, 0.02727950304226146)
(11.515151515151516, 0.027977231894550623)
(11.636363636363637, 0.028681287357186936)
(11.757575757575758, 0.02939157891076445)
(11.878787878787879, 0.030108017363066567)
(12.0, 0.030830514841134676)
};
\addlegendentry{$m=3$}
\addplot+ [mark = {none}]coordinates {
(0.0, NaN)
(0.12121212121212122, 0.0019783603272489347)
(0.24242424242424243, 9.05696920924481e-5)
(0.36363636363636365, 5.4047322425848694e-6)
(0.48484848484848486, 2.9828111386893405e-7)
(0.6060606060606061, 1.1561939623211717e-8)
(0.7272727272727273, 2.0454098665172802e-10)
(0.8484848484848485, 5.420936583378123e-13)
(0.9696969696969697, 0.0)
(1.0909090909090908, 1.9139273443933833e-15)
(1.2121212121212122, 2.2777614037771334e-12)
(1.3333333333333333, 8.483238383909738e-11)
(1.4545454545454546, 9.085189098386785e-10)
(1.5757575757575757, 5.141545384252743e-9)
(1.696969696969697, 1.9794602379172408e-8)
(1.8181818181818181, 5.897626385489717e-8)
(1.9393939393939394, 1.464956544831142e-7)
(2.0606060606060606, 3.179071512714036e-7)
(2.1818181818181817, 6.218089810332945e-7)
(2.303030303030303, 1.1203780569390363e-6)
(2.4242424242424243, 1.8892269935569126e-6)
(2.5454545454545454, 3.016717283815516e-6)
(2.6666666666666665, 4.60287356177201e-6)
(2.787878787878788, 6.758033657768996e-6)
(2.909090909090909, 9.601349008905018e-6)
(3.0303030303030303, 1.3259226876533322e-5)
(3.1515151515151514, 1.7863783592533635e-5)
(3.272727272727273, 2.355135853749605e-5)
(3.393939393939394, 3.0461122407606114e-5)
(3.515151515151515, 3.8733800525381305e-5)
(3.6363636363636362, 4.851052213429206e-5)
(3.757575757575758, 5.993179936722468e-5)
(3.878787878787879, 7.313663438476534e-5)
(4.0, 8.826174961172567e-5)
(4.121212121212121, 0.00010544093370111444)
(4.242424242424242, 0.0001248044944802653)
(4.363636363636363, 0.0001464788094665987)
(4.484848484848484, 0.0001705859643602666)
(4.606060606060606, 0.0001972434700886697)
(4.7272727272727275, 0.00022656404938299526)
(4.848484848484849, 0.00025865548440309787)
(4.96969696969697, 0.0002936205175603993)
(5.090909090909091, 0.0003315567983523462)
(5.212121212121212, 0.00037255686969366026)
(5.333333333333333, 0.0004167081878785941)
(5.454545454545454, 0.0004640931709474384)
(5.575757575757576, 0.0005147892708002805)
(5.696969696969697, 0.0005688690649541297)
(5.818181818181818, 0.0006264003643354355)
(5.9393939393939394, 0.0006874463339469676)
(6.0606060606060606, 0.00075206562366076)
(6.181818181818182, 0.0008203125067503779)
(6.303030303030303, 0.0008922370241006354)
(6.424242424242424, 0.000967885132329194)
(6.545454545454546, 0.0010472988543010087)
(6.666666666666667, 0.001130516430750574)
(6.787878787878788, 0.0012175724719213985)
(6.909090909090909, 0.001308498108306892)
(7.03030303030303, 0.0014033211397321966)
(7.151515151515151, 0.001502066182142687)
(7.2727272727272725, 0.0016047548115858642)
(7.393939393939394, 0.0017114057049740718)
(7.515151515151516, 0.0018220347772954408)
(7.636363636363637, 0.0019366553150207265)
(7.757575757575758, 0.002055278105516921)
(7.878787878787879, 0.0021779115623306693)
(8.0, 0.002304561846252715)
(8.121212121212121, 0.0024352329821176696)
(8.242424242424242, 0.0025699269713172317)
(8.363636363636363, 0.0027086439000479686)
(8.484848484848484, 0.002851382043321231)
(8.606060606060606, 0.002998137964797454)
(8.727272727272727, 0.0031489066125112036)
(8.848484848484848, 0.0033036814105757875)
(8.969696969696969, 0.003462454346961663)
(9.090909090909092, 0.003625216057441904)
(9.212121212121213, 0.0037919559058326576)
(9.333333333333334, 0.00396266206061993)
(9.454545454545455, 0.004137321568104942)
(9.575757575757576, 0.004315920422181196)
(9.696969696969697, 0.004498443630859577)
(9.818181818181818, 0.004684875279660257)
(9.93939393939394, 0.004875198591999407)
(10.06060606060606, 0.005069395986670786)
(10.181818181818182, 0.005267449132555662)
(10.303030303030303, 0.005469339000655673)
(10.424242424242424, 0.005675045913579499)
(10.545454545454545, 0.005884549592568056)
(10.666666666666666, 0.006097829202184741)
(10.787878787878787, 0.006314863392756078)
(10.909090909090908, 0.006535630340670706)
(11.030303030303031, 0.006760107786628126)
(11.151515151515152, 0.006988273071928818)
(11.272727272727273, 0.007220103172896214)
(11.393939393939394, 0.007455574733515617)
(11.515151515151516, 0.00769466409636915)
(11.636363636363637, 0.00793734733195049)
(11.757575757575758, 0.00818360026642986)
(11.878787878787879, 0.00843339850794637)
(12.0, 0.008686717471494732)
};
\addlegendentry{$m=4$}
\addplot+ [mark = {none}]coordinates {
(0.0, NaN)
(0.12121212121212122, 0.00046689104568595197)
(0.24242424242424243, 1.0509444681186078e-5)
(0.36363636363636365, 3.313447492202287e-7)
(0.48484848484848486, 9.536204892635021e-9)
(0.6060606060606061, 1.7858002739381186e-10)
(0.7272727272727273, 1.283827409973212e-12)
(0.8484848484848485, 1.0135749298930738e-15)
(0.9696969696969697, 0.0)
(1.0909090909090908, 1.5949394536611529e-16)
(1.2121212121212122, 5.0498289182365035e-15)
(1.3333333333333333, 4.326164644178182e-13)
(1.4545454545454546, 7.833624091586782e-12)
(1.5757575757575757, 6.506520023639246e-11)
(1.696969696969697, 3.3752540181735893e-10)
(1.8181818181818181, 1.2801030032651173e-9)
(1.9393939393939394, 3.887621427744924e-9)
(2.0606060606060606, 1.0010205672299234e-8)
(2.1818181818181817, 2.270296921116004e-8)
(2.303030303030303, 4.657722594659191e-8)
(2.4242424242424243, 8.812491993122846e-8)
(2.5454545454545454, 1.5599552376603286e-7)
(2.6666666666666665, 2.612127798868269e-7)
(2.787878787878788, 4.1732577808522187e-7)
(2.909090909090909, 6.404944684581502e-7)
(3.0303030303030303, 9.495136547415073e-7)
(3.1515151515151514, 1.3657819928074268e-6)
(3.272727272727273, 1.9132238540411756e-6)
(3.393939393939394, 2.6181723516880948e-6)
(3.515151515151515, 3.509221694539059e-6)
(3.6363636363636362, 4.617056477878517e-6)
(3.757575757575758, 5.97426476770056e-6)
(3.878787878787879, 7.615140975522397e-6)
(4.0, 9.575483615503752e-6)
(4.121212121212121, 1.189239218955823e-5)
(4.242424242424242, 1.460406664886938e-5)
(4.363636363636363, 1.774961216262652e-5)
(4.484848484848484, 2.1368851294264668e-5)
(4.606060606060606, 2.550214515526702e-5)
(4.7272727272727275, 3.0190224627048493e-5)
(4.848484848484849, 3.547403238459587e-5)
(4.96969696969697, 4.1394576121274064e-5)
(5.090909090909091, 4.799279312781429e-5)
(5.212121212121212, 5.530942617787857e-5)
(5.333333333333333, 6.338491050437162e-5)
(5.454545454545454, 7.225927155068095e-5)
(5.575757575757576, 8.197203305868676e-5)
(5.696969696969697, 9.2562135029792e-5)
(5.818181818181818, 0.00010406786102120578)
(5.9393939393939394, 0.00011652677422925594)
(6.0606060606060606, 0.0001299756617977254)
(6.181818181818182, 0.0001444504867896498)
(6.303030303030303, 0.00015998634725825143)
(6.424242424242424, 0.00017661744188101765)
(6.545454545454546, 0.00019437704162929043)
(6.666666666666667, 0.00021329746697071087)
(6.787878787878788, 0.00023341007012411873)
(6.909090909090909, 0.000254745221918232)
(7.03030303030303, 0.0002773323028218675)
(7.151515151515151, 0.0003011996977502378)
(7.2727272727272725, 0.0003263747942698033)
(7.393939393939394, 0.00035288398386012707)
(7.515151515151516, 0.00038075266589854127)
(7.636363636363637, 0.0004100052540831599)
(7.757575757575758, 0.0004406651850097791)
(7.878787878787879, 0.000472754928645617)
(8.0, 0.0005062960004804529)
(8.121212121212121, 0.0005413089751281607)
(8.242424242424242, 0.0005778135011879928)
(8.363636363636363, 0.0006158283171921965)
(8.484848484848484, 0.0006553712684675789)
(8.606060606060606, 0.0006964593247745351)
(8.727272727272727, 0.0007391085985803625)
(8.848484848484848, 0.0007833343638521874)
(8.969696969696969, 0.0008291510752557932)
(9.090909090909092, 0.0008765723876636832)
(9.212121212121213, 0.0009256111758846804)
(9.333333333333334, 0.000976279554530352)
(9.454545454545455, 0.001028588897955658)
(9.575757575757576, 0.0010825498601992453)
(9.696969696969697, 0.0011381723948792007)
(9.818181818181818, 0.001195465774982401)
(9.93939393939394, 0.0012544386125098944)
(10.06060606060606, 0.0013150988779386146)
(10.181818181818182, 0.0013774539194652518)
(10.303030303030303, 0.0014415104819997138)
(10.424242424242424, 0.0015072747258844364)
(10.545454545454545, 0.001574752245321322)
(10.666666666666666, 0.0016439480864801784)
(10.787878787878787, 0.001714866765279499)
(10.909090909090908, 0.0017875122848194814)
(11.030303030303031, 0.0018618881524676634)
(11.151515151515152, 0.0019379973965754954)
(11.272727272727273, 0.0020158425828291178)
(11.393939393939394, 0.002095425830226398)
(11.515151515151516, 0.0021767488266754274)
(11.636363636363637, 0.002259812844215838)
(11.757575757575758, 0.002344618753860221)
(11.878787878787879, 0.002431167040056593)
(12.0, 0.002519457814775213)
};
\addlegendentry{$m=5$}
\end{axis}

\end{tikzpicture}



==> png/qt.tex <==
\begin{tikzpicture}[]
\begin{axis}[legend pos = {north west}, xlabel = {$t$}, grid=major]\addplot+ [mark = {none}]coordinates {
(0.0, 0.0)
(0.030303030303030304, -0.006421501490296567)
(0.06060606060606061, -0.020594015654042497)
(0.09090909090909091, -0.03963463260823753)
(0.12121212121212122, -0.062008101387594924)
(0.15151515151515152, -0.08664231630084389)
(0.18181818181818182, -0.11271061766865621)
(0.21212121212121213, -0.13953952838961836)
(0.24242424242424243, -0.1665605606360794)
(0.2727272727272727, -0.19328176623425367)
(0.30303030303030304, -0.2192695075247814)
(0.3333333333333333, -0.24413606414846883)
(0.36363636363636365, -0.26753081961744923)
(0.3939393939393939, -0.2891337676342249)
(0.42424242424242425, -0.30865058850842875)
(0.45454545454545453, -0.3258088265968058)
(0.48484848484848486, -0.3403548628871165)
(0.5151515151515151, -0.3520514762746857)
(0.5454545454545454, -0.36067585005836955)
(0.5757575757575758, -0.3660179214147188)
(0.6060606060606061, -0.3678789993847488)
(0.6363636363636364, -0.3660705960894183)
(0.6666666666666666, -0.36041342942947946)
(0.696969696969697, -0.35073656526950936)
(0.7272727272727273, -0.33687667424109446)
(0.7575757575757576, -0.31867738360684056)
(0.7878787878787878, -0.2959887086296029)
(0.8181818181818182, -0.2686665509493263)
(0.8484848484848485, -0.2365722538335365)
(0.8787878787878788, -0.1995722060141143)
(0.9090909090909091, -0.15753748727987585)
(0.9393939393939394, -0.11034355015438367)
(0.9696969696969697, -0.05786993291966162)
(1.0, 0.0)
(1.0303030303030303, 0.06337929366580602)
(1.0606060606060606, 0.13237761713148466)
(1.0909090909090908, 0.20710145928110202)
(1.121212121212121, 0.28765430810345577)
(1.1515151515151516, 0.3741368152200252)
(1.1818181818181819, 0.4666469472409107)
(1.2121212121212122, 0.565280125318512)
(1.2424242424242424, 0.6701293540951114)
(1.2727272727272727, 0.7812853410927282)
(1.303030303030303, 0.8988366074671714)
(1.3333333333333333, 1.0228695909396652)
(1.3636363636363635, 1.1534687416258491)
(1.393939393939394, 1.2907166114010158)
(1.4242424242424243, 1.4346939373701835)
(1.4545454545454546, 1.585479719950432)
(1.4848484848484849, 1.743151296019459)
(1.5151515151515151, 1.907784407537492)
(1.5454545454545454, 2.079453266008551)
(1.5757575757575757, 2.2582306131107748)
(1.606060606060606, 2.4441877777935113)
(1.6363636363636365, 2.637394730110502)
(1.6666666666666667, 2.837920132033282)
(1.696969696969697, 3.0458313854665677)
(1.7272727272727273, 3.2611946776673264)
(1.7575757575757576, 3.484075024251451)
(1.7878787878787878, 3.714536309955907)
(1.8181818181818181, 3.9526413273098866)
(1.8484848484848484, 4.198451813355589)
(1.878787878787879, 4.4520284845476255)
(1.9090909090909092, 4.713431069949556)
(1.9393939393939394, 4.982718342836571)
(1.9696969696969697, 5.259948150804752)
(2.0, 5.545177444479562)
(2.0303030303030303, 5.838462304909122)
(2.0606060606060606, 6.139857969721419)
(2.090909090909091, 6.449418858118713)
(2.121212121212121, 6.767198594777052)
(2.1515151515151514, 7.093250032713945)
(2.1818181818181817, 7.427625275182729)
(2.212121212121212, 7.770375696648121)
(2.242424242424242, 8.121551962893639)
(2.272727272727273, 8.481204050308166)
(2.303030303030303, 8.849381264395703)
(2.3333333333333335, 9.226132257549553)
(2.3636363636363638, 9.611505046129315)
(2.393939393939394, 10.005547026876728)
(2.4242424242424243, 10.408304992704076)
(2.4545454545454546, 10.819825147886675)
(2.484848484848485, 11.240153122689119)
(2.515151515151515, 11.669333987453042)
(2.5454545454545454, 12.107412266172517)
(2.5757575757575757, 12.554431949581664)
(2.606060606060606, 13.010436507777511)
(2.6363636363636362, 13.475468902399918)
(2.6666666666666665, 13.949571598388994)
(2.696969696969697, 14.432786575339373)
(2.727272727272727, 14.925155338469525)
(2.757575757575758, 15.426718929223352)
(2.787878787878788, 15.937517935520278)
(2.8181818181818183, 16.457592501669282)
(2.8484848484848486, 16.986982337961315)
(2.878787878787879, 17.5257267299539)
(2.909090909090909, 18.07386454746097)
(2.9393939393939394, 18.631434253260267)
(2.9696969696969697, 19.19847391153002)
(3.0, 19.775021196025975)
};
\addlegendentry{$t^2\log(t^2)$}
\end{axis}

\end{tikzpicture}


